ReLU's Revival: On the Entropic Overload in Normalization-Free Large Language Models

LayerNorm is a critical component in modern large language models (LLMs) for stabilizing training and ensuring smooth optimization. However, it introduces significant challenges in mechanistic interpretability, outlier feature suppression, faithful signal propagation, and computational and communication complexity of private inference. This work explores desirable activation functions in normalization-free decoder-only LLMs. Contrary to the conventional preference for the GELU in transformer-based models, our empirical findings demonstrate an {\em opposite trend} -- ReLU significantly outperforms GELU in LayerNorm-free models, leading to an {\bf 8.2\%} perplexity improvement. We discover a key issue with GELU, where early layers experience entropic overload, leading to the under-utilization of the representational capacity of attention heads. This highlights that smoother activations like GELU are {\em ill-suited} for LayerNorm-free architectures, whereas ReLU's geometrical properties -- specialization in input space and intra-class selectivity -- lead to improved learning dynamics and better information retention in the absence of LayerNorm. This study offers key insights for optimizing transformer architectures where LayerNorm introduces significant challenges. The code and implementation are available at https://github.com/Nandan91/relu-revival-normfree

==> tables/3_table_ffn_lf_dr.tex <==

\begin{table}[t]
\centering
\caption{Perplexity  analysis for understanding the impact of dropping  GELUs from all FFN layers, and subsequent complexity reduction through layer fusion and then substituting them with an identity connection. An 3.2$\times$ FLOPs reduction is achieved, at the cost of a 24\% increase in perplexity, compared to standard GPT-2 model with GELUs in their FFNs. }
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccccc} \toprule 
\multirow{2}{*}{ GPT-2 configuration } & \multirow{2}{*}{GELUs} & \multirow{2}{*}{Params} & \multirow{2}{*}{FLOPs} & \multirow{2}{*}{Perplexity} & \multicolumn{2}{c}{Savings} \\
\cmidrule(lr{0.5em}){6-7} 
& & & & & Params & FLOPs \\ \toprule 
Baseline  & 4.72M & 124.2M & 10.6B & 2.69 & 1.0$\times$ & 1.0$\times$ \\
SlimGELU FFN & 0 &124.2M & 10.6B & 3.38 & 1.0$\times$ & 1.0$\times$ \\
FusedLayer FFN & 0  &74.7M & 5.1B & 3.34 & 1.7$\times$ & 2.1$\times$ \\
IdentityLink FFN & 0  &67.6M & 3.3B & 3.33 & 1.8$\times$ & 3.2$\times$ \\ \bottomrule 
\end{tabular} }
\end{table}




==> tables/4_table_WNorm_SNorm_MlpGains.tex <==
\begin{wraptable}[7]{r}{0.45\textwidth - .5\columnsep}
\centering
\vspace{-0.85\intextsep}
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{cccc} \toprule 
& WNorm & SNorm & Scaled\\ \toprule 
Eval PPL & 3.640 & 3.624 & 3.478 \\ \bottomrule 
\end{tabular} }
\vspace{-0.5em}
\caption{Perplexity comparison  of weight normalization, spectral normalization, and learnable scaling employed in FFN of softmax-only GPT-2 model.} 
\label{tab:SNormVsWNormVsMlpGains}
\end{wraptable}




==> tables/5_table_gpt2_12L_clen_128.tex <==



\begin{table}[t]
\centering
\caption{Results, and comparison against SOTA \citep{he2024simplifying}, when  GPT-2 ($L$=12, $H$=12, $d$=768) model is trained from scratch on CodeParrot \citep{codeParrot} dataset with context length  128.} \vspace{-0.7em}
\label{tab:GPT2CLen128}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{0.2cm}lclcccccc}
\toprule
& \multirow{2}[4]{*}{Network Arch.} & \multirow{2}[4]{*}{PPL} & \multirow{2}[4]{*}{\#Nonlinear Ops} & \multicolumn{2}{c}{\#FLOPs} & \multirow{2}[4]{*}{\shortstack{Comm.\\(GB)}} & \multirow{2}[4]{*}{\shortstack{Lat.\\(min.)}} & \multicolumn{2}{c}{Savings} \\
\cmidrule(lr){5-6} \cmidrule(lr){9-10}
& & & & FFN & Attn. & & & Comm. & Lat. \\
\midrule
\multirow{6}{*}{  \rotatebox[origin=c]{90}{Baseline} } & \multirow{3}{*}{${\tt SM + LN + G}$} & \multirow{3}{*}{2.69} & SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{14.5B} & \multirow{3}{*}{7.7B} & \multirow{3}{*}{25.32} & \multirow{3}{*}{8.21} & \multirow{3}{*}{1$\times$} & \multirow{3}{*}{1$\times$} \\
& & & LN:$24\times\mathbb{R}^{128\times768}$ & & & & & & \\
& & & G:$12\times\mathbb{R}^{128\times3072}$ & & & & & & \\ \cline{2-10}
& \multirow{3}{*}{${\tt SM + LN + R}$} & \multirow{3}{*}{2.76} & SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{14.5B} & \multirow{3}{*}{7.7B} & \multirow{3}{*}{9.44} & \multirow{3}{*}{6.06} & \multirow{3}{*}{2.68$\times$} & \multirow{3}{*}{1.35$\times$} \\
& & & LN:$24\times\mathbb{R}^{128\times768}$ & & & & & & \\
& & & R:$12\times\mathbb{R}^{128\times3072}$ & & & & & & \\
\midrule
\multirow{6}{*}{  \rotatebox[origin=c]{90}{SOTA} } & \multirow{2}{*}{${\tt SM + ScFFN}$} & \multirow{2}{*}{4.00} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{14.5B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.83} & \multirow{2}{*}{5.31} &  \multirow{2}{*}{3.71$\times$} & \multirow{2}{*}{1.55$\times$} \\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\ \cline{2-10}
&\multirow{2}{*}{${\tt SM + ScFuFFN}$}  & \multirow{2}{*}{3.97} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{1.8B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.31} & \multirow{2}{*}{4.50}  & \multirow{2}{*}{4.00$\times$} & \multirow{2}{*}{1.82$\times$}\\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\ \cline{2-10}
&\multirow{2}{*}{${\tt SM + ScFuFFNi_1}$}  & \multirow{2}{*}{4.00} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{1.2B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.30} & \multirow{2}{*}{4.44} & \multirow{2}{*}{4.00$\times$}  & \multirow{2}{*}{1.85$\times$} \\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\
\midrule
\multirow{5}{*}{  \rotatebox[origin=c]{90}{\bf AERO} } &${\tt SM + ScFFN}$ & 3.50 &  SM:$144\times\mathbb{R}^{128\times128}$ & 14.5B & 7.7B &  6.95 & 5.68  & 3.64$\times$ & 1.45$\times$ \\			
&${\tt SM + ScFuFFN}$ & 3.48 &  SM:$144\times\mathbb{R}^{128\times128}$ & 1.8B & 7.7B & 6.43 & 4.76  & 3.94$\times$  & 1.72$\times$ \\
&${\tt SM + ScFuFFNi_6}$ & 3.54 & SM:$144\times\mathbb{R}^{128\times128}$ & 0.9B & 7.7B  & 6.29 & 4.23  & 4.00$\times$ & 1.94$\times$ \\ \cline{2-10}
&$\text{EReg}({\tt SM(t) + ScFuFFN})$ & 3.21 &  SM:$144\times\mathbb{R}^{128\times128}$ & 1.8B & 7.7B  & 6.43 & 4.76  & 3.94$\times$ & 1.72$\times$ \\
&$\text{EReg}({\tt SM(t) + ScFuFFNi_6})$ & 3.25 & SM:$144\times\mathbb{R}^{128\times128}$ & 0.9B & 7.7B &  6.29 & 4.23 & 4.00$\times$ & 1.94$\times$ \\
\bottomrule
\end{tabular}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%

	
	
	


% & & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\

%\begin{table}[t]
%\centering
%\caption{Results on GPT2-small model on Codeparrot dataset with context length 128.}
%\begin{tabular}{lclcccccc}
%\toprule
%\multirow{2}[4]{*}{Net-config} & \multirow{2}[4]{*}{PPL} & \multirow{2}[4]{*}{\#Nonlinear Ops} & \multicolumn{2}{c}{\#FLOPs} & \multirow{2}[4]{*}{\shortstack{Comm.\\(GB)}} & \multirow{2}[4]{*}{\shortstack{Lat.\\(Sec.)}} & \multicolumn{2}{c}{Savings} \\
%\cmidrule(lr){4-5} \cmidrule(lr){8-9}
%& & & Attn & FFN & & & Comm. & Lat. \\
%\midrule
%\multirow{3}{*}{\shortstack{${\tt SM + LN + R}$\\(Baseline)}} & \multirow{3}{*}{2.69} & SM: $144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} \\
%& & LN: $24\times\mathbb{R}^{128\times768}$ & & & & & & \\
%& & G: $12\times\mathbb{R}^{128\times3072}$ & & & & & & \\
%\midrule
%\multirow{3}{*}{${\tt SM + LN + R}$} & \multirow{3}{*}{2.76} & SM: $144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} \\
%& & LN: $24\times\mathbb{R}^{128\times768}$ & & & & & & \\
%& & R: $12\times\mathbb{R}^{128\times3072}$ & & & & & & \\
%\midrule
%${\tt SM + ScFFN}$ & 3.50 & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%${\tt SM + ScFuFFN}$ & 3.48 & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%${\tt SM + ScFuFFNi_6}$ & 3.54 & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%\midrule
%\multirow{2}{*}{\shortstack{${\tt SM + ScFFN}$ \\ (SOTA \citep{he2024simplifying})}}  & \multirow{2}{*}{4.00} & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%& & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\
%\midrule
%\multirow{2}{*}{\shortstack{${\tt SM + ScFuFFN}$ \\ (SOTA \citep{he2024simplifying})}}  & \multirow{2}{*}{3.97} & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%& & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\
%\midrule
%\multirow{2}{*}{\shortstack{${\tt SM + ScFuFFNi_1}$ \\ (SOTA \citep{he2024simplifying})}}  & \multirow{2}{*}{4.00} & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%& & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\
%\midrule
%$\text{EReg}({\tt SM(t) + ScFuFFN})$ & 3.21 & SM: $144\times\mathbb{R}^{128\times128}$ & & & & & & \\
%\bottomrule
%\end{tabular}
%\end{table}




